Tree-Like Justification Systems are Consistent

Justification theory is an abstract unifying formalism that captures semantics of various non-monotonic logics. One intriguing problem that has received significant attention is the consistency problem: under which conditions are justifications for a fact and justifications for its negation suitably related. Two variants of justification theory exist: one in which justifications are trees and one in which they are graphs. In this work we resolve the consistency problem once and for all for the tree-like setting by showing that all reasonable tree-like justification systems are consistent.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{Y. Lierler, J.F. Morales, C. Dodaro, V. Dahl, M. Gebser, T. Tekle (Eds.):\\ International Conference on Logic Programming 2022 (ICLP'22).\\
EPTCS 364, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.364.1}{10.4204/EPTCS.364.1}}
\pdfoutput=1

